Mean-Covariance Steering of a Linear Stochastic System with Input Delay and Additive Noise

In this paper, we introduce a novel approach to solve the (mean-covariance) steering problem for a fairly general class of linear continuous-time stochastic systems subject to input delays. Specifically, we aim at steering delayed linear stochastic differential equations to a final desired random variable with given mean and covariance. We first establish a controllability result for these control systems, revealing the existence of a lower bound under which the covariance of the control system can not be steered. This structural threshold covariance stems from a unique combined effect due to stochastic diffusions and delays. Next, we propose a numerically cheap approach to reach any neighbor of this threshold covariance in finite time. Via an optimal control-based strategy, we enhance the aforementioned approach to keep the system covariance small at will in the whole control horizon. Under some additional assumptions on the dynamics, we give theoretical guarantees on the efficiency of our method. Finally, numerical simulations are provided to ground our theoretical findings, showcasing the ability of our methods in optimally approaching the covariance threshold.

==> 50_Old_Optimal_Control.tex <==
In the previous section, we showed the existence of tractable feedback controls that solve the steering problem. Such control laws may not guarantee that the covariance remains small during the whole control horizon $[0,T]$. In this section, our objective is to establish an efficiently implementable control strategy that keeps the state covariance consistently low along its trajectory, and not just at the final time. %Fortunately, the state's variance, a quadratic form, offers an avenue for application of the LQ framework.
%Utilizing practical numerical techniques ,
For this, we propose to compute controllers that enable approaching any neighbor of the the covariance threshold via techniques from Linear Quadratic (LQ) control \cite{yong_stochastic_1999}. The goal consists of minimizing the quadratic functional $J$\footnote{No confusion in the notation of the functional costs shall arise.}, defined as
\begin{equation}\label{eq:def_quadratic_optimal_cost_2}
\begin{split}
    J(U,X) \triangleq & \espE \left[ \int_h^T X(t)^T Q(t) X(t) dt + X(T)^T G X(T) \right] \\
    & + \espE \left[\int_0^{T-h} U(t)^T R(t) U(t) dt \right],
\end{split}
\end{equation}
where $Q \in L^\infty([0,T], \mathcal{S}_n^+)$, $G \in \mathcal{S}_n^+$ and $R \in L^\infty([0,T], \mathcal{S}_n^{++})$. This functional cost penalizes the covariance along the trajectory, the final covariance, as well as the control effort. %Note that we do not penalize the state $X$ prior to time $h$ since the control has no effect on it.
Our problem thus states:
\begin{equation}\label{eq:problem_min_cost_X}
    \min_{U \in \mathcal{U}} J(U,X), \quad \text{ $X$ follows the SDE \eqref{eq:base_system_linear_delayed_null_mean}.}
\end{equation}
%To apply non-delayed optimal control techniques, such as the ones given by \cite{yong_stochastic_1999}, 
To effectively solve \eqref{eq:problem_min_cost_X}, using equation \eqref{eq:link_artstein_original} we replace the process $X$ with the process $Y$ in $J$. The benefit of this transformation is that optimal control of non-delayed systems may be leveraged, e.g., \cite{yong_stochastic_1999}. For the first time, we compute upper bounds for $J$. %offering upper bound on the minimal variance covariance in the case of a non-time-varying dynamic.
They allow us to claim that, when the penalization on the control effort, via $R(t)$, approaches zero, the optimal controls for $J$ enable the covariance of the delayed SDE to track any neighbor of the threshold covariance.

\subsection{Optimal control of the delayed SDE.}
%Just as there exists a minimal covariance that cannot be undershot, we demonstrate the existence of a corresponding minimum variance (weighted by the matrix $Q$) that cannot be surpassed.
We may change variable in \eqref{eq:problem_min_cost_X} as follows. For $t > h$, let us denote $V_{min,Q}(t)$ the following positive real number: 
$$
V_{min,Q}(t) \triangleq \int_{t-h}^t \sigma(s)^T \Phi_A(t,s)^T Q(t) \Phi_A(t,s) \sigma(s) ds.
$$
%We can rewrite our minimization problem with the following lemma.
\begin{lemma}\label{lem:rewrite_cost_artstein_nondelayed}
The cost function $J$ can be written in terms of the state $Y$ as follows:
\begin{equation}\label{eq:def_quadratic_optimal_cost_artstein}
\begin{split}
J(U,X) & = \espE \left[ \int_0^{T-h} Y(t)^T \overline{Q}(t) Y(t) dt \right] \\
& + \espE \left[ Y(T-h)^T \overline{G} Y(T-h) \right] \\
& + \espE \left[ \int_0^{T-h} U(t)^T R(t) U(t) dt \right] \\
& + \int_h^T V_{min,Q}(t) dt + V_{min,G}(T),
\end{split}
\end{equation}
where $$\overline{Q}(t) \triangleq \Phi_A(t+h,t)^T Q(t+h) \Phi_A(t+h,t) $$ and $$\overline{G} \triangleq \Phi_A(T+h,T)^T G \Phi_A(T+h,T) $$ are symmetric positive matrices.
\end{lemma}
\begin{proof}
 Since the processes $\Phi_A(t,t-h) Y(t-h)$ and $\int_{t-h}^t \Phi_A(t,s) \sigma(s) dW_s$ are independent, similar computations to the ones in the proof of Lemma \ref{lem:relation_covariance_artstein_and_original} yield, for $t>h$
\begin{align*}
& \espE \left[ X(t)^T Q(t) X(t) \right] = \\
& \espE \left[ Y(t-h)^T \Phi_A(t,t-h)^T Q(t) \Phi_A(t,t-h) Y(t-h) \right] \\
& + \espE \left[ \left( \int_{t-h}^{t} \sigma(s) \Phi_A(t,s) dW_s \right)^T Q(t) \cdot \right. \\
& \left. \hspace{5em} \left( \int_{t-h}^{t} \sigma(s) \Phi_A(t,s) dW_s \right) \right].
\end{align*}
Therefore, by leveraging \eqref{eq:quadratic_variation_of_stochastic_integral} we may compute
\begin{align*}
\espE \left[ X(t)^T Q(t) X(t) \right] & = \espE \left[ Y(t-h)^T \overline{Q}(t-h) Y(t-h) \right] \\
& + V_{min,Q}(t).
\end{align*}
Replacing the latter formula in \eqref{eq:def_quadratic_optimal_cost_2}, %for $\espE \left[ X(t)^T Q(t) X(t) \right]$,
finally yields \eqref{eq:def_quadratic_optimal_cost_artstein}.
\end{proof}
At this step, we can apply the results from \cite[Chapter 6.2]{yong_stochastic_1999} to obtain optimal controls minimizing \eqref{eq:def_quadratic_optimal_cost_2} in the form of feedback controls:
\begin{theorem}\label{thm:analytic_solution_}
The control $U^*$ solving problem \eqref{eq:problem_min_cost_X} is given by 
\begin{equation*}
    U^* = - R(t)^{-1} \overline{B}(t)^T P(t) Y(t) ,
\end{equation*}
with $P(\cdot)$ solving the deterministic Riccati equation
\begin{equation}\label{eq:Riccati_ODE_optimal}
    \left\{
    \begin{array}{ll}
    \dot{P} & = -A^T P - P A - \overline{Q} + P \overline{B}  R^{-1} \overline{B} ^T P\\
    P(0) &= \overline{G}.
    \end{array}
    \right.
\end{equation}
\end{theorem}
\begin{proof}
Since the values of $V_{min,Q}(t)$ are independent from the control, Lemma \ref{lem:rewrite_cost_artstein_nondelayed} shows that the minimization problem \eqref{eq:problem_min_cost_X} is equivalent to the following:
\begin{equation}\label{eq:problem_min_cost_Y}
    \min_{u \in \mathcal{U}} \overline{J}(U,Y) ,
\end{equation}
where $\overline{J}$ is defined as
\begin{equation}\label{eq:def_quadratic_optimal_cost}
\begin{split}
    \overline{J}(U,Y) \triangleq & \espE \left[ \int_0^{T-h} Y(t)^T \overline{Q}(t) Y(t) dt  \right] \\
    & + \espE \left[ Y(T-h)^T \overline{G} Y(T-h)\right] \\
    & + \espE \left[ \int_0^{T-h} U(t)^T R(t) U(t) dt \right],\\
    & \quad \text{and $Y$ follows the SDE \eqref{eq:artstein_system_linear}.}
\end{split}
\end{equation}
This problem is LQ, and thus we may apply the results in \cite[Chapter 6.2]{yong_stochastic_1999} to conclude.
\end{proof}

Thanks to Lemma \ref{lem:rewrite_cost_artstein_nondelayed}, we may note that \eqref{eq:def_quadratic_optimal_cost_2} is lower-bounded by the following quantity:
\begin{equation} \label{eq:minVarTrack}
    V_{min} \triangleq \int_h^T V_{min,Q}(t) dt + V_{min,G}(T),
\end{equation}
%which is structural to the system.
As in the previous sections, we aim at developing a strategy to compute a control ensuring the covariance of delayed SDEs optimally tracks \eqref{eq:minVarTrack}. %Intuitively, by reducing the penalty matrix $R$ for the control effort, we expect to minimize the variance cost to the greatest extent.
More specifically, we will demonstrate that when $R$ tends to zero our strategy ensures that
$$
\min_{U \in \mathcal{U}} J(U,X) \underset{R \rightarrow 0}{\rightarrow} V_{min} ,
$$
meeting our desired goal.

\subsection{Upper bounds under stationary dynamics}

%Affirming that the preceding optimal controller can effectively approach the optimal lower bound of the variance is not a straightforward task. In this subsection, we demonstrate that for time-independent matrices $A$ and $B$, the computation of an optimal controller with minimal control effort penalty results in a controller that closely approaches the minimal variance bound.
%To do so, we first prove the result for controllers that are feedbacks of the state with a constant gain. 

From now on, we assume the matrices $A$ and $B$ are time-independent, and we select the specific control weight $R(t) = \rho I_d$, where $\rho > 0$ is a user-defined parameter that characterizes the control effort in \eqref{eq:def_quadratic_optimal_cost_2}. We accordingly denote the associated cost functional by $J_\rho$, which corresponds to
\begin{equation}\label{eq:def_quadratic_optimal_cost_3}
\begin{split}
    J_\rho(U,X) \triangleq & \espE \left[ \int_h^T X(t)^T Q(t) X(t) dt + X(T)^T G X(T) \right] \\
    & + \rho \ \espE \left[\int_0^{T-h} U(t)^T U(t) dt \right] .
\end{split}
\end{equation}
We denote by $U_\rho$ the corresponding optimal control, whose existence if granted by Theorem \ref{thm:analytic_solution_}, whereas $X_\rho$ denotes the corresponding state trajectory.

Our objective is to show that as $\rho$ tends to zero, the variance of $X_\rho$ tends to the threshold quantity \eqref{eq:minVarTrack}.
%\begin{equation}\label{eq:base_system_linear_delayed_stationnary}
%\left\{
%    \begin{array}{ll}
%   dX(t) &= \hspace{1em} \left( A X(t) + B U(t - h) \right) dt + \sigma(t) dW_t, \\
%    X(0) &= \hspace{1em} 0 , \\
%   U(s) &= \hspace{1em} 0 \quad \text{for } s \in [-h_d, 0[, 
%    \end{array}
%    \right.
%\end{equation}
For this, let $\lambda > 0$, and $K_\lambda$ and $H_\lambda$ be matrices such that 
$$
H_\lambda \triangleq A - \overline{B} K_\lambda, \quad \max( \Re(Sp( H_\lambda ) )) < - \lambda.
$$
Since the pair $(A,\overline{B})$ is controllable, such matrices exist thanks to the pole placement theorem, see, e.g., \cite{coron_control_2009}.
We denote by $X_\lambda$ the solution to \eqref{eq:base_system_linear_delayed_null_mean} when steered under the feedback control
$$
U_\lambda(t) = - K_\lambda Y_\lambda(t),
$$
where $Y_\lambda(t)$ is the Artstein transform of $X_\lambda$. Finally, let us denote the variance of $X(t)$ by $V_{X,Q}(t) \triangleq \espE[X(t)^T Q(t) X(t)]$, for every $t \in (h,T)$.
\begin{lemma}\label{lem:covariance_linear_feed_const_goes_zero}
If $H_\lambda$ is a normal matrix, for every $t \in (0,T)$ the following estimate holds true:
\begin{equation}\label{eq:estimate_covariance_feedback_stabilization}
V_{X_\lambda, Q}(t) - V_{min,Q}(t)  \leq  \frac{\Vert \sigma \Vert_\infty^2 \Vert Q \Vert_\infty \Vert e^{Ah} \Vert^2}{2 \lambda}
\end{equation}
\end{lemma}
\begin{proof}
If $t \in (0,T)$, thanks to Lemma \ref{lem:relation_covariance_artstein_and_original} we can write the difference between $V_{X_\lambda, Q}(t)$ and $V_{min,Q}(t)$ in terms of the covariance of $Y$ as
\begin{align*}
V_{X_\lambda, Q}(t) - V_{min,Q}(t) =  \espE [ Y(t-h)^T e^{A^Th} Q(t) e^{Ah} Y(t-h) ] . 
\end{align*}
Also, the solution $Y_\lambda$ to \eqref{eq:artstein_system_linear} under the feedback control $U_\lambda$ can be explicitly computed as
\begin{align*}
Y_\lambda(t) = \int_0^t e^{H_\lambda(t-s)} \sigma(s) dW_s .
\end{align*}
Thus, thanks to Ito's quadratic variation formula applied to $V_{Y_\lambda}$, we may compute
\begin{align*}
& V_{X_\lambda, Q}(t) - V_{min,Q}(t)  =\\
& \int_0^{t-h} \sigma(s)^T e^{H^T_\lambda(t-h-s)} ds \ e^{A^Th} Q(t) e^{Ah} e^{H_\lambda(t-h-s)} \sigma(s) ds \\
& = \int_0^{t-h} \Vert \sqrt{Q(t)} e^{Ah} e^{H_\lambda(t-h-s)} \sigma(s) \Vert^2 ds \\
& \leq \Vert Q(t) \Vert_\infty \Vert e^{Ah} \Vert^2 \int_0^{t-h} \Vert e^{H_\lambda(t-h-s)} \sigma(s) \Vert^2 ds.
\end{align*}
Since $H_\lambda$ is a normal matrix and $(t-h-s) > 0$, there holds 
$$\Vert e^{H_\lambda(t-h-s)} \sigma(s) \Vert^2 \leq \max(Sp(e^{H_\lambda(t-h-s)})) \Vert \sigma(s) \Vert^2 ,$$
\textcolor{red}{Here's I guess how you can remove the normality assumption. Let $r = (t-h-s)$ and $H_\lambda(r) = V(r) J(r) V(r)^{-1}$ be the Jordan decomposition. Thus,
\begin{align*}
    &\Vert e^{H_\lambda(r)} \sigma(s) \Vert^2 \le \| V(r) \exp( J(r) ) V(r)^{-1} \|^2_F \| \sigma(s) \|^2 \\
    &= \textnormal{tr}( (V(r) \exp( J(r) ) V(r)^{-1})^{\top} V(r) \exp( J(r) ) V(r)^{-1} ) \| \sigma(s) \|^2 \\
    &= \textnormal{tr}( V(r)^{-1}(V(r) \exp( J(r) ) V(r)^{-1})^{\top} V(r) \exp( J(r) ) ) \| \sigma(s) \|^2 \\
    &\le \textnormal{tr}( V(r)^{-1}(V(r) \exp( J(r) ) V(r)^{-1})^{\top} V(r) ) \textnormal{tr}( \exp( J(r) ) ) \| \sigma(s) \|^2 \\
    &= \textnormal{tr}( (V(r) \exp( J(r) ) V(r)^{-1})^{\top} V(r) V(r)^{-1} ) \textnormal{tr}( \exp( J(r) ) ) \| \sigma(s) \|^2 \\
    &= \textnormal{tr}( (V(r) \exp( J(r) ) V(r)^{-1})^{\top} ) \textnormal{tr}( \exp( J(r) ) ) \| \sigma(s) \|^2 \\
    &= \dots \\
    &= \textnormal{tr}( \exp( J(r) ) )^2 \| \sigma(s) \|^2 \\
    &\le C(n) \max \exp(\lambda(H_{\lambda}(r)))^2 \| \sigma(s) \|^2 ,
\end{align*}
and you conclude.}

from which we conclude that
\begin{align*}
& V_{X_\lambda, Q}(t) - V_{min,Q}(t) \\
& \leq \Vert Q \Vert_\infty \Vert e^{Ah} \Vert^2  \Vert \sigma \Vert_\infty^2 \int_0^{t-h} e^{-\lambda(t-h-s)}   ds \\
& \leq  \frac{\Vert \sigma \Vert_\infty^2 \Vert Q \Vert_\infty \Vert e^{Ah} \Vert^2}{2 \lambda}.
\end{align*}
%\textcolor{red}{Bloquage ici, dans ma preuve j'ai utilisé une égalité fausse (Spectre($A^T A$) est TRES différent de Spectre($A^2$) ), j'ai essayé de trouver un autre moyen de me ramener au spectre mais sans succès}
\end{proof}
This result may be adjusted to non-normal $H_\lambda$ matrices, using density arguments or the fact that $H_\lambda$ is similar to a normal matrix. \textcolor{red}{You should not need this anymore.}

\begin{theorem}
The following converge holds true:
\begin{equation}
    J_\rho( U_\rho ) \underset{\rho \rightarrow 0}{ \rightarrow} \int_h^T V_{min,Q}(t) dt + V_{min,G}(T)
\end{equation}
\end{theorem}
\begin{proof}
The control effort $\int_0^{T-h} U_\lambda(t)^T U_\lambda(t) dt$ tends to $\infty$ when $\lambda$ tends to $\infty$. \textcolor{red}{A détailler?} If we take $\rho_\lambda$ such that $\rho_\lambda \int_0^{T-h} U_\lambda(t)^T U_\lambda(t) dt$ tends to 0 when $\lambda$ tends to $\infty$ then $\rho_\lambda$ tends to 0 \textcolor{red}{What you need this latter information for?}. 
Therefore, thanks to Lemma \ref{lem:covariance_linear_feed_const_goes_zero} we may compute
\begin{align*}
    J_{\rho_\lambda} & (U_\lambda) = \int_h^T V_{X_\lambda,Q}(t) dt + V_{X_\lambda,G}(T) \\
    & + \rho_\lambda \int_0^{T-h} U_\lambda(t)^T U_\lambda(t) dt \\
    & \underset{\lambda \rightarrow \infty}{\rightarrow} \int_h^T V_{min,Q}(t) dt + V_{min,G}(T) .
\end{align*}
But $U_{\rho_\lambda}$ is optimal control, and thus $J_{\rho_\lambda}( U_{\rho_\lambda} ) \leq J_{\rho_\lambda}( U_\lambda )$. In particular, $J_{\rho_\lambda}( U_{\rho_\lambda} )$ also converges to \eqref{eq:minVarTrack} when $\lambda \to \infty$. Since $\textcolor{red}{\lambda \to J_{\rho_\lambda}( U_{\rho_\lambda} )}$ \textcolor{red}{Is this correct?} is an increasing function, we conclude the above limit is the unique existing limit for $\rho \to 0$.
\end{proof}
This lemma shows the optimal control-based strategy can also attain the minimal covariance, if the penalization on the control effort is sufficiently relaxed.

\textcolor{red}{UNCLEAR: COMMENTER LE THEOREME}

\textcolor{red}{AJOUTER TRANSITION, DIRE QU'ON VÉRIFIE LE THÉORÈME A TRAVERS LES SIMUS}





